On the optimality of sliced inverse regression in high dimensions

The central subspace of a pair of random variables $(y,x) \in \mathbb{R}^{p+1}$ is the minimal subspace $\mathcal{S}$ such that $y \perp \hspace{-2mm} \perp x\mid P_{\mathcal{S}}x$. In this paper, we consider the minimax rate of estimating the central space of the multiple index models $y=f(\beta_{1}^{\tau}x,\beta_{2}^{\tau}x,...,\beta_{d}^{\tau}x,\epsilon)$ with at most $s$ active predictors where $x \sim N(0,I_{p})$. We first introduce a large class of models depending on the smallest non-zero eigenvalue $\lambda$ of $var(\mathbb{E}[x|y])$, over which we show that an aggregated estimator based on the SIR procedure converges at rate $d\wedge((sd+s\log(ep/s))/(n\lambda))$. We then show that this rate is optimal in two scenarios: the single index models; and the multiple index models with fixed central dimension $d$ and fixed $\lambda$. By assuming a technical conjecture, we can show that this rate is also optimal for multiple index models with bounded dimension of the central space. We believe that these (conditional) optimal rate results bring us meaningful insights of general SDR problems in high dimensions.

==> frontmatter.tex <==
\begin{frontmatter}

\title{On the optimal rate of estimating the central subspace }
\runtitle{SIR-minimax }
\thankstext{t1}{Qian}

\begin{aug}
  \author{\fnms{Qian} \snm{Lin}\thanksref{m1}\ead[label=e1]{qianlin@cmsa.fas.harvard.edu}\thanksref{t1}}

   \runauthor{Q. Lin}
  \affiliation{Harvard University\thanksmark{m1} }
  \address{Qian Lin\\
    Center of Mathematical Sciences\\
     and Applications \\
    Harvard University\\
    One Oxford Street \\
    Cambridge, MA 02138  \\
    USA\\
    \printead{e1}}    
\end{aug}

\begin{abstract}
 The subspace $\mathcal{S}$ is called the central subspace of $(y,\vx)$, if it is the minimal subspace such that $y\independent \vx | P_{\mathcal{S}}\vx$. Looking for the central subspace is commonly referred to as {\it `sufficient dimension reduction'} (SDR). 
Sliced inverse regression (SIR) is arguably one of the most commonly used sufficient dimension reduction algorithm with a wide range of applications. We consider the minimax estimation of the central space in high dimensional setting. Assuming the dimension $d$ of central space is fixed, the linearity condition and coverage condition, we establish the optimal rates of convergence for estimating 	the central space  under mild conditions. The lower bound is obtained by an application of Fano's lemma. . We also make a speculation when $d$ is diverging at moderate rate.


\end{abstract}

\begin{keyword}%[class=AMS]
\kwd{dimension reduction space}
\kwd{optimal rates}
\kwd{sliced inverse regression}
\kwd{semi-definite positive programming}
\end{keyword}
\end{frontmatter}

==> header.tex <==
\usepackage{amsgen,amsmath,amstext,amsbsy,amsopn,amssymb,amscd,amsthm,lipsum}
\usepackage{color,graphicx,verbatim,multirow}
\usepackage{url,caption, subcaption}
\setlength{\topmargin}{-0.5in}
\setlength{\oddsidemargin}{0in}
\setlength{\evensidemargin}{0in}
\setlength{\textheight}{9in}
\setlength{\textwidth}{6.5in}
\setlength{\footskip}{0.2in}



\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{example}{Example}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{remark}{Remark}[section]
%\newtheorem{conjecture}{Conjecture}[section]


\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\corref}[1]{Corollary~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand{\figref}[1]{Figure~\ref{#1}}

%% \input{mathsymbol.tex}
